Cryo-Near-Field Photovoltage Microscopy of Heavy-Fermion Twisted Symmetric Trilayer Graphene

Ever since the initial experimental observation of correlated insulators and superconductivity in the flat Dirac bands of magic angle twisted bilayer graphene, a search for the microscopic description that explains its strong electronic interactions has begun. While the seemingly disagreeing electronic transport and scanning tunneling microscopy experiments suggest a dichotomy between local and extended electronic orbitals, definitive experimental evidence merging the two patterns together has been much sought after. Here, we report on the local photothermoelectric measurements in the flat electronic bands of twisted symmetric trilayer graphene (TSTG). We use a cryogenic scanning near-field optical microscope with an oscillating atomic force microscopy (AFM) tip irradiated by the infrared photons to create a nanoscopic hot spot in the planar samples, which generates a photocurrent that we probe globally. We observe a breakdown of the non-interacting Mott formalism at low temperatures (10K), signaling the importance of the electronic interactions. Our measurements reveal an overall negative offset of the Seebeck coefficient and significant peaks of the local photovoltage values at all positive integer fillings of the TSTG's moir\'e superlattice, further indicating a substantial deviation from the classical two-band semiconductor Seebeck response. We explain these observations using the interacting topological heavy-fermion model. In addition, our data reveal a spatial variation of the relative interaction strength dependent on the measured local twist angle (1.2{\deg} - 1.6{\deg}). Our findings provide experimental evidence of heavy fermion behaviour in the topological flat bands of moir\'e graphene and epitomize an avenue to apply local thermoelectric measurements to other strongly correlated materials in the disorder-free limit.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
